What can LLM tell us about cities?

This study explores the capabilities of large language models (LLMs) in providing knowledge about cities and regions on a global scale. We employ two methods: directly querying the LLM for target variable values and extracting explicit and implicit features from the LLM correlated with the target variable. Our experiments reveal that LLMs embed a broad but varying degree of knowledge across global cities, with ML models trained on LLM-derived features consistently leading to improved predictive accuracy. Additionally, we observe that LLMs demonstrate a certain level of knowledge across global cities on all continents, but it is evident when they lack knowledge, as they tend to generate generic or random outputs for unfamiliar tasks. These findings suggest that LLMs can offer new opportunities for data-driven decision-making in the study of cities.

==> bak/bak_exp_full.tex <==
\begin{table*}[ht]
    \centering
    \caption{Overall Result: Knowledge in the City }
    \begin{tabularx}{\textwidth}{lXXXXXXXXX}
    % \begin{tabular}{|c|c|c|c|c|c|c|c|}
        \toprule
        \textbf{City} & \textbf{Data} & \textbf{Features} & \textbf{Target} & \textbf{Location only} & \textbf{Direct Ask} & \textbf{AvgY}\\
        \midrule
        \multirow{3}{*}{\textbf{New York}} & Pickup & \textbf{1.469} & 1.611 &1.597 & 3.114 & 1.654  \\
        & Dropoff & \textbf{1.689}  &1.784 &1.743  & 3.952  &1.794 \\
        & Crime & \textbf{1.850} &2.164 & 2.122 &  3.466& 1.898\\
        & 311 & \textbf{1.836} & 1.853  & 1.892 & 4.430 & 2.187 \\
        \midrule

        \multirow{2}{*}{\textbf{Chicago}} & Pickup & \textbf{1.821}  &1.956 & 1.935 & 3.189   & 1.962  \\
        & Dropoff & \textbf{1.745}  & 1.957 &1.993  &3.450  &2.017 \\
        & Crime & \textbf{1.304} & 2.261 & 2.135 &  3.153 & 2.265\\
        \midrule

        \multirow{2}{*}{\textbf{Washington DC}} & Pickup & \textbf{1.891} &1.946 & 1.954 &3.019  & 1.972  \\
        & Dropoff & \textbf{1.849}  &1.897 & 1.849 &3.200  & 1.888 \\
        & Crime &1.898  & \textbf{1.897} &2.210  &5.194  & 2.345 \\
        \midrule

        \multirow{1}{*}{\textbf{Austin}} & 311 & 1.751 & 1.669 & \textbf{1.613} & 4.191 & 2.565  \\

        \midrule
        
        \multirow{2}{*}{\textbf{Cincinnati}} & Crime &1.598 &1.785 & \textbf{1.205}  & 4.701 &  1.735\\
        &311  & \textbf{2.088} & 2.156 & 2.389 & 5.028 & 2.779 \\
        % \midrule

        % \multirow{2}{*}{\textbf{Fort-Worth}} & Crime & & &  &  &  \\
        % &311  &  &  &  &  &  \\

        \bottomrule
    % \end{tabular}
    \end{tabularx}
    \label{table:overall_result_regions}
\end{table*}



\begin{table*}[ht]
    \centering
    \caption{Overall Result: City-Level Knowledge }
    \resizebox{1.0\linewidth}{!}{
    \renewcommand{\arraystretch}{1.0}
    \begin{tabular}{|c|c|c|c|c|c|c|c|}
    % \begin{tabularx}{\textwidth}{lXXXXXXX}
        \toprule
        \textbf{Category} & \textbf{Data} & \textbf{Coverage} & \textbf{Features} & \textbf{Target} & \textbf{Location only} & \textbf{Direct Ask} & \textbf{AvgY} \\
        \midrule

        \multirow{4}{*}{\textbf{Air Quality}} & $NO_2[\mu g/m^3]$ & 749 cities in Europe & \textbf{3.350} & 4.369 & 4.454 & 4.526 &  4.552 \\
        & $O_3[\mu g/m^3]$ & 749 cities in Europe & \textbf{1187.053} & 1468.872 & 1365.309 & 3995.112 & 1606.761 \\
        & $PM_{10}[\mu g/m^3]$ & 749 cities in Europe & 4.196 & 4.643 & 4.903 & \textbf{3.869} & 5.554 \\
        & $PM_{2.5}[\mu g/m^3]$ &  749 cities in Europe & 3.586 & 3.514 & 3.618 & \textbf{2.162} & 4.127 \\
        \midrule
        
        \multirow{4}{*}{\textbf{Energy}} 
        & Water Withdrawal [100 million $m^3$] & 391 cities in China  & \textbf{13.396} &15.567 &15.666 &17.384&15.779  \\
        &Total Energy Consumption[10Kt-coal]& 331 cities in China& \textbf{918.499} & 1434.635& 1362.503&1208.621 &1265.201 \\
        &Traditional Energy Consumption[10Kt-coal] &331 cities in China &\textbf{894.514} &1399.252 &1353.043 &4177.396 &1168.283\\
        &Renewable Energy Consumption[10Kt-coal] &331 cities in China &\textbf{468.813} &642.317 &787.872 &4682.0557 &472.219\\
        \midrule

        
        \multirow{4}{*}{\textbf{Industry}} 
        & Total [100 million Yuan] & 245 cities in China  & \textbf{3357.649} & 5040.151&4689.549 &3508.391 &5296.166  \\
        & Mining [100 million Yuan] & 245 cities in China & \textbf{314.635} & 344.956& 340.588&329.822 &324.143 \\
        & Manufacture [100 million Yuan] & 245 cities in China & \textbf{3224.627} & 4735.158& 4422.688&3383.922 &5010.069 \\
        & Utilities [100 million Yuan] & 245 cities in China & \textbf{309.551} & 314.225& 351.839&372.218&378.266 \\
        \midrule

        
        \multirow{4}{*}{\textbf{Environment}} 
        & $CO_2$ Emission[Mt$CO_2$] & 343 cities globally & \textbf{10.195}   &13.409  &14.794 & 13.365& 12.507   \\
        & Livestock Methane Emissions[t] & 347 cities in China & \textbf{24654.910} & 28534.404 & 28168.048 & 45339.452 & 35258.758 \\
        & $CO_2$ Emission[kg-$CO_2$/cap] & 52 cities in Japan & \textbf{139.980}   &181.923  &188.248 & 853.416& 170.185   \\
        & $CO_2$ Emission[Mt-$CO_2$] & 82 regions in Russia & \textbf{23.673}   &28.638  &26.049 & 23.962& 25.605   \\        
        \midrule

        \multirow{5}{*}{\textbf{Health}} &  Dengue & 1541 cities globally & 1858.819 & 1459.020 & \textbf{1439.626} & 3309.807 & 1947.404\\
        &  COVID-19 & 415 counties in US & 2234.806 & 2367.352 & 2400.570 & \textbf{2159.229} & 2784.648\\
        %&  Chinese thermal comfort & 49 Chinese cities &  14.317 & 14.324 & \textbf{13.884} & 17.814 & 15.075\\
        &  life expectancy & 29 England cities & \textbf{2.587} & 2.613 & 2.659 & 13.098 & 2.897\\
        & Access to Healthy Assets and Hazards&374 districts in UK &\textbf{5.384} &7.019 &7.238 &16.386 & 6.191  \\
        \midrule

        \multirow{2}{*}{\textbf{Traffic}} & Average travel time per 10 km[s] & 387 cities globally & \textbf{205.524} & 228.385 & 238.750 & 370.434 & 269.465\\
         & Average speed in rush hour[km/h] & 387 cities globally & \textbf{7.048} & 8.098 & 8.338 & 10.436 & 10.016 \\ 
        \midrule

        \multirow{3}{*}{\textbf{Transportation}} & PNT level at 500m[\%] & 85 cities globally & \textbf{10.535}& 11.085 & 10.306 & 14.269 & 14.159 \\
        & PNT level at 1000m[\%] & 85 cities globally & \textbf{13.223} & 15.525 & 14.501 & 19.412 & 20.194 \\
        & PNT level at 1500m[\%] & 85 cities globally & \textbf{13.976} & 17.940 & 16.115 & 19.918 & 22.549 \\
        \midrule

        \multirow{1}{*}{\textbf{Material}} & Material stocks[tonnes/capital] & 337 cities in China & \textbf{33.706} & 34.244 & 35.029 & 106.679 & 36.601 \\
        \midrule
        
        \multirow{2}{*}{\textbf{Innovation}} 
         & Notable People (since 1900) & 237 countries globally& \textbf{16294.750}  &16916.926&17269.500&16519.245 &16926.415\\
         & Patent (2014) & 487 cities globally& \textbf{2490.455}  &2851.428&2874.744&3305.860 &2826.339\\
         \midrule
         
        \multirow{2}{*}{\textbf{Economy}} & Built-up-area[square kilometer] & 49 states in USA & \textbf{581.526} & 669.044 &642.068 & 587.556 & 613.266 \\
        & Average Home value[thousand dollars] & 200 cities in USA & 184.324 & 223.657 &203.369 & \textbf{23.961} & 238.022 \\
        
        \bottomrule
    \end{tabular}
    }
    % \end{tabularx}
    \label{table:overall_result_cities}
\end{table*}

==> bak/case_study.tex <==
\subsection{Case Study: function features in RGB }

This case study explores the application of LLM in analyzing the features of residential, commercial, and recreational areas across 255 zones in NYC. We use the GPT-4o model to extract the residential, commercial, and recreation features of each taxi zone in New York City, quantifying these features on a scale from 0 to 255. Residential areas are represented in red, commercial areas in green, and recreational areas in blue. We then create an RGB map of New York City in Figure~\ref{fig:NYC_RGB} to study the characteristics of urban zoning.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.48\textwidth]{figure/NYC_RGB.png}
    \caption{RGB Map of New York City Boroughs (Red: Residential, Green: Commercial, Blue: Recreation)}
    \label{fig:NYC_RGB}
\end{figure}

Through the visualization shown in Figure~\ref{fig:NYC_RGB}, several key insights were identified:

\begin{enumerate}
\item \textbf{Residential Dominance}: Certain zones, primarily in the outer boroughs, exhibited a high concentration of residential areas. These areas were marked in red and indicated zones where housing developments are the primary land use.
\item \textbf{Commercial Hubs}: The commercial areas, highlighted in green, were predominantly located in Manhattan and parts of Brooklyn and Queens. These areas are characterized by a high density of businesses and commercial activities.
\item \textbf{Recreational Spaces}: Recreational zones, shown in blue, were more evenly distributed across NYC, with notable concentrations in parks and waterfront areas. These zones provide vital green spaces for community activities and environmental sustainability.

\end{enumerate}

Transferring this method, we can create an RGB map for any city in the world. This map will simply and intuitively show the characteristics of different city zones.




\subsection{Case Study: Chicago Nightlife}
\begin{figure}[h]
    \centering
    \includegraphics[width=0.48\textwidth]{figure/poi-dist7.pdf}
    \caption{Chicago Nightlife}
    \label{fig:chicago_night}
\end{figure}


==> bak/exp-bigtable-bk.tex <==


\begin{table*}[]
\resizebox{1.0\linewidth}{!}{
\renewcommand{\arraystretch}{1.4}
\begin{tabular}{c|c|r|l|l|r|r|r|r}
\toprule
                  \multicolumn{2}{l|}{{ \textbf{Category}}}    &  \textbf{ID}                               & \textbf{Data}                            & \textbf{Coverage}             & \textbf{Exp Feature}     & \textbf{Imp Feature}            &  \textbf{No Feature} & \textbf{Direct Ask} \\ \hline
     & { }      & {{ 1}}  & { NO₂ {[}µg/m³{]}}                                & {{ 749 cities, Europe}}      & { \textbf{3.35}}     & {{ 4.369}}     & { 4.552}     & { 4.526}               \\ \cline{3-9} 
     & { }      & {{ 2}}  & { O₃ {[}µg/m³{]}}                                 & {{ 749 cities, Europe}}      & { \textbf{1187.053}} & {{ 1468.872}}  & { 1606.761}  & { 3995.1}              \\ \cline{3-9} 
     & { }      & {{ 3}}  & { PM₁₀ {[}µg/m³{]}}                               & {{ 749 cities, Europe}}      & { 4.196}             & {{ 4.643}}     & { 5.554}     & { \textbf{3.869}}      \\ \cline{3-9} 
     & { }      & {{ 4}}  & { PM₂.₅ {[}µg/m³{]}}                              & {{ 749 cities, Europe}}      & { 3.586}             & {{ 3.514}}     & { 4.127}     & { \textbf{2.162}}      \\ \cline{3-9} 
     & { }      & {{ 5}}  & { CO₂ Emission {[}MtCO₂{]}}                       & {{ 343 cities globally}}       & { \textbf{10.257}}   & {{ 13.409}}    & { 12.507}    & { 13.365}              \\ \cline{3-9} 
     & { }      & {{ 6}}  & { Livestock Methane Emissions {[}t{]}}            & {{ 347 cities, China}}       & { \textbf{24654.91}} & {{ 28534.404}} & { 35258.758} & { 45339}               \\ \cline{3-9} 
     & { }      & {{ 7}}  & { CO₂ Emission {[}kg-CO₂/cap{]}}                  & {{ 52 cities, Japan}}        & { \textbf{139.98}}   & {{ 181.923}}   & { 170.185}   & { 853.42}              \\ \cline{3-9} 
     & { }      & {{ 8}}  & { CO₂ Emission {[}Mt-CO₂{]}}                      & {{ 82 regions, Russia}}      & { \textbf{23.673}}   & {{ 28.638}}    & { 25.605}    & { 23.962}              \\ \cline{3-9} 
     & \multirow{-9}{*}{{ \textbf{\rotatebox{90}{Environment}}}}    & {{ 9}}  & { Water Withdrawal {[}100 million m³{]}}          & {{ 391 cities, China}}       & { \textbf{13.396}}   & {{ 15.567}}    & { 15.779}    & { 17.384}              \\ \cline{2-9} 
     & { }      & {{ 10}} & { Total Energy {[}10Kt-coal{]}}       & {{ 331 cities, China}}       & { \textbf{886.745}}  & {{ 1400.858}}  & { 1250.447}  & { 1208.014}              \\ \cline{3-9} 
     & { }      & {{ 11}} & { Traditional Energy {[}10Kt-coal{]}} & {{ 331 cities, China}}       & { \textbf{851.103}}  & {{ 1293.122}}  & {1154.6094}  & { 2250.133}              \\ \cline{3-9} 
     & \multirow{-3}{*}{{ \textbf{\rotatebox{90}{Energy}}}}       & {{ 12}} & { Renewable Energy  {[}10Kt-coal{]}}   & {{ 331 cities, China}}       & { \textbf{110.72}}  & {{ 135.49}}   & { 143.639}   & { 2934.214}              \\ \cline{2-9} 
     & { }      & {{ 13}} & { Dengue}     & {{ 1541 cities globally}}      & { \textbf{ 1858.819}}          & {1896.265}   & { 1947.404}  & { 3309.8}              \\ \cline{3-9} 
     & { }      & {{ 14}} & { COVID-19}   & {{ 415 counties, US}}        & { 2234.806}          & {{ 2367.352}}  & { 2784.648}  & { \textbf{2159.2}}     \\ \cline{3-9} 
     & { }      & {{ 15}} & { Life Expectancy}                                & {{ 29 cities, England}}      & { \textbf{2.587}}    & {{ 2.613}}     & { 2.897}     & { 13.098}              \\ \cline{3-9} 
     & \multirow{-4}{*}{{\textbf{\rotatebox{90}{Health}}}}        & {{ 16}} & { Access to Healthy Assets}           & {{ 374 districts, UK}}       & { \textbf{5.384}}    & {{ 7.019}}     & { 6.191}     & { 16.386}              \\ \cline{2-9} 
     & { }      & {{ 17}} & { Average travel time per 10 km {[}s{]}}          & {{ 387 cities globally}}       & { \textbf{205.524}}  & {{ 228.385}}   & { 269.465}   & { 370.43}              \\ \cline{3-9} 
     & { }      & {{ 18}} & { Avg speed {[}km/h{]}}          & {{ 387 cities globally}}       & { \textbf{7.048}}    & {{ 8.098}}     & { 10.016}    & { 10.436}              \\ \cline{3-9} 
     & { }      & {{ 19}} & { PNT level at 500m {[}\%{]}}                     & {{ 85 cities globally}}        & { \textbf{10.535}}   & {{ 11.085}}    & { 14.159}    & { 14.269}              \\ \cline{3-9} 
     & { }      & {{ 20}} & { PNT level at 1000m {[}\%{]}}                    & {{ 85 cities globally}}        & { \textbf{13.223}}   & {{ 15.525}}    & { 20.194}    & { 19.412}              \\ \cline{3-9}  
     & \multirow{-5}{*}{{ \textbf{\rotatebox{90}{Transport}}}} & {{ 21}} & { PNT level at 1500m {[}\%{]}}                    & {{ 85 cities globally}}        & { \textbf{13.976}}   & {{ 17.94}}     & { 22.549}    & { 19.918}              \\ \cline{2-9} 
     & { }      & {{ 22}} & { Total {[}100 million Yuan{]}}                   & {{ 245 cities, China}}       & { \textbf{3357.649}} & {{ 5040.151}}  & { 5296.166}  & { 3508.4}              \\ \cline{3-9} 
     & { }      & {{ 23}} & { Mining {[}100 million Yuan{]}}                  & {{ 245 cities, China}}       & { \textbf{314.635}}  & {{ 344.956}}   & { 324.143}   & { 329.82}              \\ \cline{3-9} 
     & { }      & {{ 24}} & { Manufacture {[}100 million Yuan{]}}             & {{ 245 cities, China}}       & { \textbf{3224.627}} & {{ 4735.158}}  & { 5010.069}  & { 3383.9}              \\ \cline{3-9} 
     & \multirow{-4}{*}{{ \textbf{\rotatebox{90}{Industry}}}}       & {{ 25}} & { Utilities {[}100 million Yuan{]}}               & {{ 245 cities, China}}       & { \textbf{309.551}}  & {{ 314.225}}   & { 378.266}   & { 372.22}              \\ \cline{2-9} 
     & { }      & {{ 26}} & { Patent}     & {{ 487 cities globally}}       & { \textbf{2490.455}} & {{ 2851.428}}  & { 2826.339}  & { 3305.9}              \\ \cline{3-9} 
     & { }      & {{ 27}} & {Home value {[}thousand dollars{]}}      & {{ 200 cities, USA}}         & { 184.324}           & {{ 223.657}}   & { 238.022}   & { \textbf{23.961}}     \\ \cline{3-9} 
\multirow{-28}{*}{\rotatebox{90}{\textbf{City Level}}}            & \multirow{-3}{*}{{ \textbf{\rotatebox{90}{Develop}}}}    & {{ 28}} & { Material stocks {[}tonnes/capital{]}}           & {{ 337 cities, China}}       & { \textbf{33.706}}   & {{ 34.244}}    & { 36.601}    & { 106.68}              \\ \hline
     & { }      & {{29}}               & NYC Pickup                        & {{ 256 regions}}        & \textbf{1.469}                           & {1.611}                            & 1.654                            & 3.114  \\ \cline{3-9} 
     & { }      & {{ 30}} & NYC Dropoff                       & {{ 256 regions}}        & \textbf{1.689}                           & {1.784}                            & 1.794                            & 3.952  \\ \cline{3-9} 
     & { }      & {{ 31}} & Chicago Pickup                    & {{ 167 regions}}    & \textbf{1.821}                           & {1.956}                            & 1.962                            & 3.189  \\ \cline{3-9} 
     & { }      & {{ 32}} & Chicago Dropoff                   & {{ 167 regions}}    & \textbf{1.745}                           & {1.957}                            & 2.017                            & 3.45   \\ \cline{3-9} 
     & { }      & {{ 33}} & DC Pickup                         & {{ 129 regions}}         & \textbf{1.891}                           & {1.946}                            & 1.972                            & 3.019  \\ \cline{3-9} 
     & \multirow{-6}{*}{{ \textbf{\rotatebox{90}{Transport}}}} & {{ 34}} & DC Dropoff                        & {{ 129 regions}}         & \textbf{1.849}                           & {1.897}                            & 1.888                            & 3.2    \\ \cline{2-9} 
     & { }      & {{ 35}} & NYC Crime                         & {{ 177 regions}}        & \textbf{1.85}                            & {2.164}                            & 1.898                            & 3.466  \\ \cline{3-9} 
     & { }      & {{ 36}} & Chicago Crime                     & {{ 77 regions}}    & \textbf{1.304}                           & {2.261}                            & 2.265                            & 3.153  \\ \cline{3-9} 
     & { }      & {37}               & DC Crime                          & {{ 41 regions}}         & 1.898& {\textbf{1.897}}                   & 2.345                            & 5.194  \\ \cline{3-9} 
     & \multirow{-4}{*}{{ \textbf{\rotatebox{90}{Crime}}}}          & {{ 38}} & Cincinnati Crime                  & {{ 67 regions}} & \textbf{1.598}& {1.785}                            & 1.735                            & 4.701  \\ \cline{2-9} 
     & { }      & {{ 39}} & NYC                               & {{ 177 regions}}        & \textbf{1.836}                           & {1.853}                            & 2.187                            & 4.43   \\ \cline{3-9} 
     & { }      & {{ 40}} & Austin                            & {{ 69 regions}}     & 1.751& \textbf{1.669}                            & 2.565                            & 4.191  \\ \cline{3-9} 
\multirow{-13}{*}{\rotatebox{90}{\textbf{Region level}}} & \multirow{-3}{*}{{ \textbf{\rotatebox{90}{311}}}}            & {{41}}               & Cincinnati                        & {{ 47 regions}} & \textbf{2.088}                           & {2.156}                            & 2.779                            & 5.028  \\ \bottomrule
\end{tabular}
}
\caption{Results on City level and Region level tasks for xxx cities over the world.}
\label{tab:overall-results}
\end{table*}



==> bak/exp.tex <==

\section{Experiment}
\subsection{Experimental Settings}
Data normalization was applied to scale all district-level target \ref{table:overall_result_regions} to a range of 0.0 to 10.0, ensuring that the data were on a comparable scale. The LLM-extracted features were similarly scaled from 0.0 to 10.0 to maintain consistency in feature representation. The LLM-generated hidden state features were limited to 32 dimensions, allowing for a manageable yet informative feature set. For evaluation, we used the Root Mean Square Error (RMSE) as the primary metric to assess the accuracy of the predictions. The machine learning model employed includes Decision Tree, Random Forest, Gradient Boosting, XGBoost, AdaBoost, and Linear Regressor. The LLM model used for hidden state method was LLaMA 3.1 8B instruct, an open-source language model allowing us to obtain the hidden states. The experiment followed a 5-fold cross-validation approach to ensure that the results were reliable and generalizable.

\subsection{Compared Methods}
\begin{itemize}
    \item \textbf{Features}: Use ChatGPT-4o to extract features from city or district data and applied various machine learning methods to predict the target.
    \item \textbf{Target}: Employed LLaMA 3.1 8B instruct to extract features from hidden state related to the target variable.
    \item \textbf{Location Only}: Used LLaMA 3.1 8B instruct to extract features from hidden state based solely on the location information.
    \item \textbf{Direct Ask}: Directly asked ChatGPT-4o for predictions on the target variable without further processing.
    \item \textbf{AvgY}: Used the average value of the target as the predicted value, serving as a baseline for comparison.
\end{itemize}

% \begin{itemize}
%     \item Data Normalization: 0.0-10.0
%     \item Scale of Human Selected Features: 0.0-10.0
%     \item Number of Hidden State Features: 32
%     \item Evaluation Metrics: Rooted Mean Square Error
%     \item ML model: Gradient Boosting
%     \item LLM model: llama 3.1 8B instruct
%     \item Train/test: 5-fold
% \end{itemize}

\subsection{Overall Result}

In this section, we conduct experiments on two-levels of data, regions-in-the-city level (noted as "region level" afterwards) and global city level (noted as "city level" afterwards). The results on xxx cities and xxx tasks are shown in Table~\ref{tab:overall-results}. The results demonstrate that the Exp Feature method, which combines LLM feature extraction with machine learning, outperforms other methods across most tasks. The Direct Ask method often shows the highest errors, indicating limitations in LLMs’ direct responses regarding specific quantitative targets. The No Feature method using the average of the training set target values, serving as a baseline, generally performs worse than Exp feature methods. This suggests that while LLMs hold substantial knowledge about cities which may help to obtain more accurate predictions. Meanwhile, Exp feature outperforms Imp feature which extract features from LLM in a hidden state format. This exhibits the necessity of explicitly finding out the related explicit features and extracting them respectively.

% \begin{enumerate}
%     \item Feature: Using LLM to extract features about a city and applying machine learning (ML) to predict the target.
%     \item Target: Using the hidden state of the LLM to ask about the task in the city and extract features.
%     \item Location Only: Using the hidden state of the LLM to ask about the city to extract features.
%     \item Direct Ask: Directly asking the LLM about the target.
%     \item AvgY: Using the average value of the target as the predicted value.
% \end{enumerate}

\subsection{Verification on Prediction Pipeline}

When queried the response for a target, LLM is likely to output meaningless generic values, which need to be differentiated from meaningful extracted features. We here present some observations on determining how to detect the meaningless outputs.

% \subsubsection{VER-I: Direct Ask LLM may return meaningless results.} The Kolmogorov-Smirnov (KS) test, kernal density estimation (KDE) and cumulative distribution (CDF) are used to compare the distribution of the extracted values with that of the ground truth values. A high KS statistic and a low p-value suggest that the LLM’s outputs significantly differ from the ground truth, possibly indicating a lack of context-specific estimation. Through the results shown in Table~\ref{} and Figure~\ref{}, we can observe that, in the COVID task, the extracted data aligns well with the groundtruth data in distribution, while in the MINING task, the extracted data deviates far from the groundtruth data in distribution.

% \begin{table}[H]
% \centering
% \caption{KS test on the predicted and groundtruth values for the COVID and MINING task.}
% \begin{tabular}{|l|c|c|}
% \hline
% \textbf{Task}                & \textbf{KS statistic} & \textbf{p-value} \\ \hline
% COVID             & 0.1518           & 0.0001       \\ \hline
% MINING             & 0.5306           & 0.0000      \\ \hline
% \end{tabular}
% \label{tab:model_performance}
% \end{table}


% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.35\textwidth]{figure/covid_error.png}
%     \caption{Covid}
%     \label{fig:covid_error}
% \end{figure}

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.35\textwidth]{figure/mining_error.png}
%     \caption{Mining}
%     \label{fig:mining_error}
% \end{figure}



% \paragraph{Definition:}
% The KS statistic is the maximum absolute difference between the ECDFs of the two datasets. It is given by:
% \[
% D = \sup_x | F_1(x) - F_2(x) |
% \]
% where \( F_1(x) \) and \( F_2(x) \) are the ECDFs of the prediction and ground truth, respectively.


% Visual tools such as kernel density estimates (KDE) plots, and cumulative distribution function (CDF) plots are used to compare the distributions of predicted and ground truth values and help identify discrepancies and biases in the LLM’s predictions.

% \textsc{Good Case: COVID}


% Kolmogorov-Smirnov Test: 

% Statistic = 0.15180722891566265

% p-value = 0.00013691683274525288

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.35\textwidth]{figure/covid_error.png}
%     \caption{Covid}
%     \label{fig:covid_error}
% \end{figure}

% \textsc{Bad Case: Industry(Mining)}


% Kolmogorov-Smirnov Test: 

% Statistic = 0.5306122448979592

% p-value = 6.639265697800818e-32


\subsubsection{VER-I: Detecting consistent generic values}  If the LLM frequently produces the same rounded number, such as 50, across various contexts, it suggests that the model may lack specific knowledge about the data in question. This behavior indicates a tendency to default to a generic or placeholder value rather than providing a contextually informed estimate.


\begin{figure}[H]
    \centering
    \includegraphics[width=0.45\textwidth]{figure/VER-1.png}
    \caption{Mining}
    \label{fig:VER-II-1}
\end{figure}
    
\subsubsection{VER-II: Detecting inconsistent values among multiple generations}: The temperature parameter of an LLM influences the degree of randomness in its outputs. If the model’s outputs display considerable variability, it suggests that the model may be uncertain about the information and is generating responses based on guesswork rather than a solid knowledge of the data. Such inconsistency indicates that the LLM may not be reliably estimating the information, instead oscillating between generic or uncertain predictions.

\begin{figure}[H]
    \centering
    \includegraphics[width=0.45\textwidth]{figure/VER-2.png}
    \caption{Water}
    \label{fig:VER-II-2}
\end{figure}




\subsection{Ablation Study}

% \begin{itemize}
%     \item use external features, like poi for taxi, census for crime
%     \item different ML models
%     \item different LLM models (chatGPT, llama)
% \end{itemize}


% \textbf{What affects the results of the feature extraction?}
% \begin{itemize}
%     % feature --  yaochen
%     % \item feature: adding explanation helps (+ ablation) % yaochen
%     \item feature values variance, +-1, relative order maintains 
    
%     % \item synonyms, similar values
%     \item language: different languages, different values
% \end{itemize}

In this section, we explore the impact of different LLMs and feature extraction techniques on the extraction results and prediction results.

\subsubsection{AS-I: Does the LLM source matter?}
We select the NYC 311 dataset\cite{NYC311_2023} and China's annual livestock methane emissions dataset\cite{city_methane} to evaluate the performance of different LLM models in feature extraction tasks. In addition, a set of random features (denoted as random feature) are used as a control group. The experimental results (shown in Table~\ref{tab:model_performance} ) demonstrate that GPT-4o exhibits best or second best performance on both datasets. This phenomenon is consistently observed among various datasets. Hence, we adopt GPT4o as the default model for all other experiments. Although Qwen2 and DeepSeek are trained with a significant amount of Chinese data, their performance on China's annual livestock methane emissions dataset does not surpass other models. 

\begin{table}[tbph]
\centering
\caption{Performance comparison across models on NYC 311 and Chain methane emissions datasets.}
\renewcommand{\arraystretch}{1.4}
\begin{tabular}{l|c|c}
\toprule
\textbf{Model}                & \textbf{NYC 311} & \textbf{Methane} \\ \hline
gpt4o                        & 1.836            & \textbf{24654.910} \\ \hline
claude3.5-sonnet             & \textbf{1.803}   & 26610.090        \\ \hline
Qwen2-72B-Instruct           & 1.971            & 29364.221        \\ \hline
deepseek-chat                & 1.946            & 28310.989        \\ \hline
llama3.1-70b-instruction      & 2.158            & 26086.093        \\ \hline
llama3.1-8b-instruction      & 2.097            & 33070.858        \\ \hline
random feature [0.0-10.0]    & \textcolor{red}{2.262}  & \textcolor{red}{35783.344} \\ \hline
avgY (no train)              & 2.187            & 35258.758        \\ \bottomrule
\end{tabular}
\label{tab:model_performance}
\end{table}

We further conduct experiments to compare two different sizes of the LLaMA3.1-Instruct model (8b and 70b) in processing specific prompts, using the last hidden state as a feature for training results measured by RMSE. The experiment utilized the NYC 311 dataset and evaluated model performance through a five-fold experiment. The results indicate that while the 70b model outperformed the 8b model in certain instances, the performance differences between the two models are not significant and varied with repeated experiments. Therefore, selecting a larger hidden layer does not always lead to significant performance improvements, and model selection should be balanced according to specific task requirements and computational resources.

% \begin{itemize}
%     \item local only prompt: Provide me with information about zip code: \{zip\_code\} of \{city\} in \{country\}.
%     \item target prompt: Provide me with information on factors that could affect 311 Service Requests in \{zip\_code\} of \{city\} in \{country\}.
%     \item data: NYC 311
% \end{itemize}

\begin{table}[H]
\centering
\caption{Comparison of three times running of LLaMA3.1-Instruct Models (8b vs. 70b) using RMSE on NYC 311 Dataset}
\renewcommand{\arraystretch}{1.4}
\begin{tabular}{c|c|c}
\toprule
\textbf{Times} & \textbf{Model}              & \textbf{Imp Feature} \\ \hline
\textbf{1}     & LLaMA3.1-8b-instruct                      & 1.806           \\ \cline{2-3} 
               & LLaMA3.1-70b-instruct                  & 1.893           \\ \cline{2-3} 
               & \textbf{Improvement (\%)}      & \textbf{-4.5\%} \\ \hline
\textbf{2}     & LLaMA3.1-8b-instruct                    & 1.892           \\ \cline{2-3} 
               & LLaMA3.1-70b-instruct                    & 1.981           \\ \cline{2-3} 
               & \textbf{Improvement (\%)}        & \textbf{-4.4\%} \\ \hline
\textbf{3}     & LLaMA3.1-8b-instruct                     & 1.971           \\ \cline{2-3} 
               & LLaMA3.1-70b-instruct                   & 1.903           \\ \cline{2-3} 
               & \textbf{Improvement (\%)}       & \textbf{3.5\%}  \\ \bottomrule
\end{tabular}

\end{table}

\subsubsection{AS-II: Does language matter in extracting features? }
\begin{table}[!t]
\centering
\caption{Language(English vs Chinese) Comparison on Different Tasks}
\renewcommand{\arraystretch}{1.4}
\begin{tabular}{c|cc|cc}
\toprule
\textbf{Task} & \multicolumn{2}{c|}{\textbf{Material stocks}}            & \multicolumn{2}{c}{\textbf{PNT level at 1500m}}\\ \cline{1-5} 
            \textbf{Prompt}          & \textbf{English }   & \textbf{Chinese}  & \textbf{English }  & \textbf{Chinese} \\ \hline
Exp Feature              & {33.706}           & \textbf{33.216} & {\textbf{13.976}} & 15.522                              \\ \hline
Imp Feature                & {\textbf{34.244}}  & 36.366          & {\textbf{17.940}} & 20.962                              \\ \hline
% Location Only         & {\textbf{35.029}}  & 35.236          & {\textbf{16.115}} & 18.443                              \\ \hline
Direct Ask            & {\textbf{106.679}} & 140.827         & {\textbf{19.918}} & 21.645                              \\ \hline
No Feature              & {36.601}  & 36.601          & {22.549}          & 22.549                              \\ \bottomrule
\end{tabular}
\label{tab:language}
\end{table}

In this study, we conduct two experiments to compare the performance of using English and Chinese languages for feature extraction on two datasets (one of the original dataset is compiled in Chinese). The results are shown in Table~\ref{tab:language}. The Chinese prompts are generated by translating the original English prompts using GPT-4o. It is shown that English prompts yield significantly better performance than Chinese prompts, even when dealing with tasks centered on Chinese cities. This outcome highlights the critical role of the corpus in determining performance, suggesting that the quality and relevance of the training data may have a more substantial impact than the language of the prompt itself. These findings provide strong evidence that a well-curated and comprehensive corpus can transcend language barriers, ensuring better results regardless of the language used in the prompts.

% \subsubsection{AS-III:  Does variance matter in extracting features? }
% In this experiment, we conducted feature extraction on the Chinese total energy consumption dataset~\cite{yang_comprehensive_2024} five times to evaluate the impact of the variance in LLM extraction results on the RMSE. The variance\_RMSE was calculated using the first extraction as the baseline. For each feature, the RMSE was computed relative to the corresponding feature in the first extraction, and the average RMSE across all features was obtained. The target\_RMSE represents the target RMSE obtained after applying the features in a machine learning model.
% \begin{table}[H]
%     \centering
%     \caption{Results of Feature Extraction Instances with variance\_RMSE and target\_RMSE values.}
%     \begin{tabular}{c|c|c}
%         \toprule
%             \textbf{Feature Extraction} & \textbf{variance\_RMSE} & \textbf{target\_RMSE} \\ \hline
%             Instance 1                           & N/A                     & 1027.160              \\ \hline
%             Instance 2                           & 0.526                   & 1032.212              \\ \hline
%             Instance 3                           & 0.557                   & 981.363               \\ \hline
%             Instance 4                           & 0.566                   & 1011.693              \\ \hline
%             Instance 5                           & 0.591                   & 929.323               \\ \hline
%             \textit{AvgY}                        & N/A                     & 1265.201              \\ \bottomrule
%         \end{tabular}
    
%     \label{table:variance}
% \end{table} 
% Despite the variance in the extracted features, the results consistently outperformed baseline AvgY.




\begin{table*}[]
\resizebox{1.0\linewidth}{!}{
\renewcommand{\arraystretch}{1.4}
\begin{tabular}{c|c|r|l|l|r|r|r|r}
\toprule
                  \multicolumn{2}{l|}{{ \textbf{Category}}}    &  \textbf{ID}                               & \textbf{Data}                            & \textbf{Coverage}             & \textbf{Exp Feature}     & \textbf{Imp Feature}            &  \textbf{No Feature} & \textbf{Direct Ask} \\ \hline
     & { }      & {{ 1}}  & { NO₂ {[}µg/m³{]}}                                & {{ 749 cities, Europe}}      & { \textbf{3.35}}     & {{ 4.369}}     & { 4.552}     & { 4.526}               \\ \cline{3-9} 
     & { }      & {{ 2}}  & { O₃ {[}µg/m³{]}}                                 & {{ 749 cities, Europe}}      & { \textbf{1187.053}} & {{ 1468.872}}  & { 1606.761}  & { 3995.1}              \\ \cline{3-9} 
     & { }      & {{ 3}}  & { PM₁₀ {[}µg/m³{]}}                               & {{ 749 cities, Europe}}      & { 4.196}             & {{ 4.643}}     & { 5.554}     & { \textbf{3.869}}      \\ \cline{3-9} 
     & { }      & {{ 4}}  & { PM₂.₅ {[}µg/m³{]}}                              & {{ 749 cities, Europe}}      & { 3.586}             & {{ 3.514}}     & { 4.127}     & { \textbf{2.162}}      \\ \cline{3-9} 
     & { }      & {{ 5}}  & { CO₂ Emission {[}MtCO₂{]}}                       & {{ 343 cities globally}}       & { \textbf{10.257}}   & {{ 13.409}}    & { 12.507}    & { 13.365}              \\ \cline{3-9} 
     & { }      & {{ 6}}  & { Livestock Methane Emissions {[}t{]}}            & {{ 347 cities, China}}       & { \textbf{24654.91}} & {{ 28534.404}} & { 35258.758} & { 45339}               \\ \cline{3-9} 
     & { }      & {{ 7}}  & { CO₂ Emission {[}kg-CO₂/cap{]}}                  & {{ 52 cities, Japan}}        & { \textbf{139.98}}   & {{ 181.923}}   & { 170.185}   & { 853.42}              \\ \cline{3-9} 
     & { }      & {{ 8}}  & { CO₂ Emission {[}Mt-CO₂{]}}                      & {{ 82 regions, Russia}}      & { \textbf{23.673}}   & {{ 28.638}}    & { 25.605}    & { 23.962}              \\ \cline{3-9} 
     & \multirow{-9}{*}{{ \textbf{\rotatebox{90}{Environment}}}}    & {{ 9}}  & { Water Withdrawal {[}100 million m³{]}}          & {{ 391 cities, China}}       & { \textbf{13.396}}   & {{ 15.567}}    & { 15.779}    & { 17.384}              \\ \cline{2-9} 
     & { }      & {{ 10}} & { Total Energy {[}10Kt-coal{]}}       & {{ 331 cities, China}}       & { \textbf{886.745}}  & {{ 1400.858}}  & { 1250.447}  & { 1208.014}              \\ \cline{3-9} 
     & { }      & {{ 11}} & { Traditional Energy {[}10Kt-coal{]}} & {{ 331 cities, China}}       & { \textbf{851.103}}  & {{ 1293.122}}  & {1154.6094}  & { 2250.133}              \\ \cline{3-9} 
     & \multirow{-3}{*}{{ \textbf{\rotatebox{90}{Energy}}}}       & {{ 12}} & { Renewable Energy  {[}10Kt-coal{]}}   & {{ 331 cities, China}}       & { \textbf{110.72}}  & {{ 135.49}}   & { 143.639}   & { 2934.214}              \\ \cline{2-9} 
     & { }      & {{ 13}} & { Dengue}     & {{ 1541 cities globally}}      & { \textbf{ 1858.819}}          & {1896.265}   & { 1947.404}  & { 3309.8}              \\ \cline{3-9} 
     & { }      & {{ 14}} & { COVID-19}   & {{ 415 counties, US}}        & { 2234.806}          & {{ 2367.352}}  & { 2784.648}  & { \textbf{2159.2}}     \\ \cline{3-9} 
     & { }      & {{ 15}} & { Life Expectancy}                                & {{ 29 cities, England}}      & { \textbf{2.587}}    & {{ 2.613}}     & { 2.897}     & { 13.098}              \\ \cline{3-9} 
     & \multirow{-4}{*}{{\textbf{\rotatebox{90}{Health}}}}        & {{ 16}} & { Access to Healthy Assets}           & {{ 374 districts, UK}}       & { \textbf{5.384}}    & {{ 7.019}}     & { 6.191}     & { 16.386}              \\ \cline{2-9} 
     & { }      & {{ 17}} & { Average travel time per 10 km {[}s{]}}          & {{ 387 cities globally}}       & { \textbf{205.524}}  & {{ 228.385}}   & { 269.465}   & { 370.43}              \\ \cline{3-9} 
     & { }      & {{ 18}} & { Avg speed {[}km/h{]}}          & {{ 387 cities globally}}       & { \textbf{7.048}}    & {{ 8.098}}     & { 10.016}    & { 10.436}              \\ \cline{3-9} 
     & { }      & {{ 19}} & { PNT level at 500m {[}\%{]}}                     & {{ 85 cities globally}}        & { \textbf{10.535}}   & {{ 11.085}}    & { 14.159}    & { 14.269}              \\ \cline{3-9} 
     & { }      & {{ 20}} & { PNT level at 1000m {[}\%{]}}                    & {{ 85 cities globally}}        & { \textbf{13.223}}   & {{ 15.525}}    & { 20.194}    & { 19.412}              \\ \cline{3-9}  
     & \multirow{-5}{*}{{ \textbf{\rotatebox{90}{Transport}}}} & {{ 21}} & { PNT level at 1500m {[}\%{]}}                    & {{ 85 cities globally}}        & { \textbf{13.976}}   & {{ 17.94}}     & { 22.549}    & { 19.918}              \\ \cline{2-9} 
     & { }      & {{ 22}} & { Total {[}100 million Yuan{]}}                   & {{ 245 cities, China}}       & { \textbf{3357.649}} & {{ 5040.151}}  & { 5296.166}  & { 3508.4}              \\ \cline{3-9} 
     & { }      & {{ 23}} & { Mining {[}100 million Yuan{]}}                  & {{ 245 cities, China}}       & { \textbf{314.635}}  & {{ 344.956}}   & { 324.143}   & { 329.82}              \\ \cline{3-9} 
     & { }      & {{ 24}} & { Manufacture {[}100 million Yuan{]}}             & {{ 245 cities, China}}       & { \textbf{3224.627}} & {{ 4735.158}}  & { 5010.069}  & { 3383.9}              \\ \cline{3-9} 
     & \multirow{-4}{*}{{ \textbf{\rotatebox{90}{Industry}}}}       & {{ 25}} & { Utilities {[}100 million Yuan{]}}               & {{ 245 cities, China}}       & { \textbf{309.551}}  & {{ 314.225}}   & { 378.266}   & { 372.22}              \\ \cline{2-9} 
     & { }      & {{ 26}} & { Patent}     & {{ 487 cities globally}}       & { \textbf{2490.455}} & {{ 2851.428}}  & { 2826.339}  & { 3305.9}              \\ \cline{3-9} 
     & { }      & {{ 27}} & {Home value {[}thousand dollars{]}}      & {{ 200 cities, USA}}         & { 184.324}           & {{ 223.657}}   & { 238.022}   & { \textbf{23.961}}     \\ \cline{3-9} 
\multirow{-28}{*}{\rotatebox{90}{\textbf{City Level}}}            & \multirow{-3}{*}{{ \textbf{\rotatebox{90}{Develop}}}}    & {{ 28}} & { Material stocks {[}tonnes/capital{]}}           & {{ 337 cities, China}}       & { \textbf{33.706}}   & {{ 34.244}}    & { 36.601}    & { 106.68}              \\ \hline
     & { }      & {{29}}               & NYC Pickup                        & {{ 256 regions}}        & \textbf{1.469}                           & {1.611}                            & 1.654                            & 3.114  \\ \cline{3-9} 
     & { }      & {{ 30}} & NYC Dropoff                       & {{ 256 regions}}        & \textbf{1.689}                           & {1.784}                            & 1.794                            & 3.952  \\ \cline{3-9} 
     & { }      & {{ 31}} & Chicago Pickup                    & {{ 167 regions}}    & \textbf{1.821}                           & {1.956}                            & 1.962                            & 3.189  \\ \cline{3-9} 
     & { }      & {{ 32}} & Chicago Dropoff                   & {{ 167 regions}}    & \textbf{1.745}                           & {1.957}                            & 2.017                            & 3.45   \\ \cline{3-9} 
     & { }      & {{ 33}} & DC Pickup                         & {{ 129 regions}}         & \textbf{1.891}                           & {1.946}                            & 1.972                            & 3.019  \\ \cline{3-9} 
     & \multirow{-6}{*}{{ \textbf{\rotatebox{90}{Transport}}}} & {{ 34}} & DC Dropoff                        & {{ 129 regions}}         & \textbf{1.849}                           & {1.897}                            & 1.888                            & 3.2    \\ \cline{2-9} 
     & { }      & {{ 35}} & NYC Crime                         & {{ 177 regions}}        & \textbf{1.85}                            & {2.164}                            & 1.898                            & 3.466  \\ \cline{3-9} 
     & { }      & {{ 36}} & Chicago Crime                     & {{ 77 regions}}    & \textbf{1.304}                           & {2.261}                            & 2.265                            & 3.153  \\ \cline{3-9} 
     & { }      & {37}               & DC Crime                          & {{ 41 regions}}         & 1.898& {\textbf{1.897}}                   & 2.345                            & 5.194  \\ \cline{3-9} 
     & \multirow{-4}{*}{{ \textbf{\rotatebox{90}{Crime}}}}          & {{ 38}} & Cincinnati Crime                  & {{ 67 regions}} & \textbf{1.598}& {1.785}                            & 1.735                            & 4.701  \\ \cline{2-9} 
     & { }      & {{ 39}} & NYC                               & {{ 177 regions}}        & \textbf{1.836}                           & {1.853}                            & 2.187                            & 4.43   \\ \cline{3-9} 
     & { }      & {{ 40}} & Austin                            & {{ 69 regions}}     & 1.751& \textbf{1.669}                            & 2.565                            & 4.191  \\ \cline{3-9} 
\multirow{-13}{*}{\rotatebox{90}{\textbf{Region level}}} & \multirow{-3}{*}{{ \textbf{\rotatebox{90}{311}}}}            & {{41}}               & Cincinnati                        & {{ 47 regions}} & \textbf{2.088}                           & {2.156}                            & 2.779                            & 5.028  \\ \bottomrule
\end{tabular}
}
\caption{Results on City level and Region level tasks for xxx cities over the world.}
\label{tab:overall-results}
\end{table*}






\input{case_study}





\subsection{Other Experiments}




% \begin{table}[h!]
%     \centering
%     \begin{tabular}{>{\bfseries}l>{\bfseries}l r r r}
%         \toprule
%         & & \textbf{no feature} & \textbf{no weekday} & \textbf{weekday} \\
%         \midrule
%         \multirow{3}{*}{\textbf{Pickup}} & \textbf{NYC} & 1.468 & \textbf{1.390} & 1.445 \\
%         & \textbf{Chicago} & 2.305 & 1.898 & \textbf{1.871} \\
%         & \textbf{DC} & 2.270 & 2.221 & \textbf{1.830} \\
%         \midrule
%         \multirow{3}{*}{\textbf{Dropoff}} & \textbf{NYC} & 1.765 & \textbf{1.510} & 1.587 \\
%         & \textbf{Chicago} & 2.250 & 1.802 & \textbf{1.786} \\
%         & \textbf{DC} & 2.484 & 2.318 & \textbf{1.975} \\
%         \bottomrule
%     \end{tabular}
%     \caption{zero-shot for Taxi Pickup and Dropoff (RMSE)}
% \end{table}

\newpage



==> bak/takeaways.tex <==
\newpage
\section{Key Takeaways}

\textit{Q1: What does LLM know?} 
\textit{A1: LLM can answer widely recognized data correctly, but can also generate random guesses. Here we show observations on how to differentiate these answers. }

\textbf{Answering widely recognized data accurately.} During the experiments, it is observed that large language models exhibit a profound understanding of widely recognized target data such as PM2.5 levels and COVID-19 statistics, resulting in exceptionally low RMSE when directly asking for these data points. This high accuracy is attributable to the extensive pre-training of LLMs on vast corpus that likely include substantial information on these popular topics. Consequently, the raw data regarding PM2.5 and COVID-19, often embedded within the training datasets, enables the LLMs to provide precise and reliable outputs. This inherent knowledge embedded in the pre-trained models underscores the capability of LLMs to serve as effective tools for accessing pre-existing data in various domains, demostraing the utility of LLMs in automating the extraction of meaningful city features, enhancing the depth and breadth of urban data analysis.

\textbf{Generate random estimates.} In instances where the LLM has not been exposed to specific data during its pre-training phase or when the required data is not readily available, the model tends to generate generic or estimated values. For example, when queried about less common or unfamiliar targets, the LLM might produce fallback estimates such as 500, 1500, or 5000. These values represent the model's best guess based on patterns it has observed in similar contexts, rather than precise or data-driven outputs. This limitation uncovers the dependency of LLMs on their training data and emphasize the need for consideration of the context to ensure the reliability of the extracted information.


\textbf{LLMs generate variable outputs for unknown data, even with low temperature settings.}
When the temperature parameter is set to a very low value such as 0.01, the LLM should show deterministic behavior, consistently outputting the same result when it has been exposed to and learned the relevant data during its pre-training. This low temperature minimizes randomness and ensures that the most probable response is selected each time. However, in cases where the LLM lacks specific knowledge about the data, even a low temperature setting like 0.01 cannot guarantee identical outputs across different instances. This could be attributed to the tiny amount of randomness involved in sampling from the probability distribution, but it is more likely because the model must rely on its generalized understanding and inference capabilities, leading to variations in its responses as it attempts to generate reasonable answers based on limited information. Therefore, the consistency of the outputs is dependent on the extent of the model’s pre-trained knowledge on the queried data.

\textbf{LLMs struggle with inference and data manipulation tasks.} Despite its vast knowledge, LLM is notably weak in inference and data manipulation tasks. Even with techniques like chain-of-thought prompting, which aims to improve the logical flow and reasoning in responses, LLM struggle to perform complex inferential tasks and accurate data manipulations. The performance can be inconsistent and unreliable when required to process and manipulate data or execute multi-step logical reasoning. 






\textit{Q2: How to use LLM to assist prediction? } \textit
{A2: Use it to generate features and train a separate prediction model to boost the prediction. Here we compare different ways of extracting features. }

\textbf{LLMs hold substantial implicit knowledge about cities. }
Taking advantage of this knowledge through feature extraction and subsequent machine learning yields the most accurate predictions.

Our method uses LLM for feature extraction and traditional machine learning models for inference and data manipulation. This hybrid approach capitalizes on the extensive knowledge embedded within LLMs, eliminating the need to gather large datasets typically required in traditional machine learning. By extracting rich, high-level features from the LLM and feeding them into machine learning models, we can achieve reliable prediction, overcoming the weaknesses of LLM in reasoning and complex data processing.

\begin{itemize}
    % manual feature is better
    \item hidden state vs. features: manually feature selection (main result)
    \item features by human knowledge vs. gpt knowledge, example in temperature in dengue, age in covid, 311 gdp crime (+examples)
\end{itemize}


\textit{Q3: What affects the results of the feature extraction?}
\textit{A3: We should carefully extracting the features, otherwise features can "lie". Here we show some factors that affect the feature extraction accuracy.}
\begin{itemize}
    % feature --  yaochen
    % \item feature: adding explanation helps (+ ablation) % yaochen
    \item feature values variance, +-1, relative order maintains 
% yaochen
    
    % \item synonyms, similar values
    \item language: different languages, different values
\end{itemize}

\textbf{Despite the variance in the extracted features, the results consistently surpassed the baseline AvgY.}
This indicates that, even though there were differences in the features obtained from multiple extractions, the method's performance remained robust. The results not only remained stable but also consistently exceeded the baseline performance metric (AvgY), demonstrating the effectiveness and reliability of the feature extraction process in capturing relevant information for the predictive task.

\textbf{LLMs emphasize that the role of the corpus outweighs the language of the prompt.}
LLMs possess advanced capabilities in multilingual processing, allowing them to seamlessly extract and interpret information from a corpus, no matter the language of the prompt. Therefore, even in tasks focused on Chinese cities, using English prompts yielded better overall results than using Chinese prompts. This validates the rationale for using English prompts in global datasets.This proficiency ensures that the underlying data is accurately understood and utilized, regardless of whether the prompt is in English, Chinese, or any other language, demonstrating the model's versatility and effectiveness in handling diverse linguistic inputs.

% \textit{Q4: Does the LLM source matter?}
% \textit{A4: Yes. Here we show the impact of using different LLMs on the final prediction results.}

% model -- zhixue

\subsubsection{AS I:} In this experiment, we evaluated different models' feature extraction capabilities using the NYC 311 dataset and China's annual livestock methane emissions dataset. Results showed that GPT-4o outperformed other models, including Qwen2 and DeepSeek, which despite their extensive training on Chinese data, did not surpass GPT-4o, suggesting its generalizable effectiveness for broader applications.
    
\subsubsection{AS II:} The experiment comparing 8b and 70b LLaMA3.1-Instruct models on the NYC 311 dataset showed that while the 70b model sometimes outperformed the 8b, the differences were not consistently significant.  This indicates that larger model sizes do not always lead to better performance, highlighting the need to balance model selection with task requirements and computational resources.




% \begin{itemize}
%     % direct ask -- zhuoheng
%     % \item popular target (pm2.5, covid), known
%     % \item unknown, direct ask: 150, 1500, 150000
%     % \item unknown, when temperature is low (0.01), random results
    
%     % \item direct ask: cannot do the inference by llm (known x --> y), chain-of-thought does not work (+ example)
%     % \item when do we know whether LLM knows this answer?
% \end{itemize}



==> checklist.tex <==
\section*{Reproducibility Checklist}

Unless specified otherwise, please answer “yes” to each question if the relevant information is described either in the paper itself or in a technical appendix with an explicit reference from the main paper. If you wish to explain an answer further, please do so in a section titled “Reproducibility Checklist” at the end of the technical appendix.

\smallskip \noindent
This paper:

\begin{itemize}
    \item Includes a conceptual outline and/or pseudocode description of AI methods introduced. \underline{yes}

    \item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results. \underline{yes}

    \item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper. \underline{yes}
\end{itemize}

\smallskip \noindent
Does this paper make theoretical contributions? \underline{no}

\smallskip \noindent
If yes, please complete the list below.

\begin{itemize}
    \item All assumptions and restrictions are stated clearly and formally. (yes/partial/no)

    \item All novel claims are stated formally (e.g., in theorem statements). (yes/partial/no)

    \item Proofs of all novel claims are included. (yes/partial/no)

    \item Proof sketches or intuitions are given for complex and/or novel results. (yes/partial/no)

    \item Appropriate citations to theoretical tools used are given. (yes/partial/no)

    \item All theoretical claims are demonstrated empirically to hold. (yes/partial/no/NA)

    \item All experimental code used to eliminate or disprove claims is included. (yes/no/NA)
\end{itemize}

\smallskip \noindent
Does this paper rely on one or more datasets? \underline{yes}

\smallskip \noindent
If yes, please complete the list below.

\begin{itemize}
    \item A motivation is given for why the experiments are conducted on the selected datasets. \underline{yes}
    
    \item All novel datasets introduced in this paper are included in a data appendix. \underline{yes}
    
    \item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. \underline{yes}

    \item All datasets drawn from the existing literature (potentially including authors' own previously published work) are accompanied by appropriate citations. \underline{yes}
    
    \item  All datasets drawn from the existing literature (potentially including authors' own previously published work) are publicly available. \underline{yes}

    \item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisfying. \underline{yes}
\end{itemize}

\smallskip \noindent
Does this paper include computational experiments? \underline{yes}

\smallskip \noindent
If yes, please complete the list below.

\begin{itemize}
    \item Any code required for pre-processing data is included in the appendix. \underline{yes}

    \item All source code required for conducting and analyzing the experiments is included in a code appendix. \underline{yes}

    \item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. \underline{yes}

    \item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from. \underline{yes}

    \item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. \underline{yes}

    \item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. \underline{yes}

    \item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. \underline{yes}

    \item This paper states the number of algorithm runs used to compute each reported result. \underline{yes}

    \item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. \underline{yes} 

    \item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). \underline{yes}

    \item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper's experiments. \underline{yes}

    \item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. \underline{yes}
\end{itemize}
    
